Observing gravitational-wave transient GW150914 with minimal assumptions

The gravitational-wave signal GW150914 was first identified on Sept 14 2015 by searches for short-duration gravitational-wave transients. These searches identify time-correlated transients in multiple detectors with minimal assumptions aboutthe signal morphology, allowing them to be sensitive to gravitational waves emitted by a wide range of sources including binary black-hole mergers. Over the observational period from September 12th to October 20th 2015, these transient searches were sensitive to binary black-hole mergers similar to GW150914 to an average distance of $\sim 600$ Mpc. In this paper, we describe the analyses that first detected GW150914 as well as the parameter estimation and waveform reconstruction techniques that initially identified GW150914 as the merger of two black holes. We find that the reconstructed waveform is consistent with the signal from a binary black-hole merger with a chirp mass of $\sim 30 \, M_\odot$ and a total mass before merger of $\sim 70 \, M_\odot$ in the detector frame.

==> Makefile <==
all: GW150914_burst.pdf

GW150914_burst.pdf: GW150914_burst.tex bwb.tex cwb.tex \
	data.tex discussion.tex introduction.tex mdc.tex \
	olib.tex pe.tex defs.tex  GW150914_burst.bib 

	pdflatex GW150914_burst.tex
	bibtex GW150914_burst
	pdflatex GW150914_burst.tex
	pdflatex GW150914_burst.tex


